Algorithmic Writing Assistance on Jobseekers' Resumes Increases Hires

There is a strong association between the quality of the writing in a resume for new labor market entrants and whether those entrants are ultimately hired. We show that this relationship is, at least partially, causal: a field experiment in an online labor market was conducted with nearly half a million jobseekers in which a treated group received algorithmic writing assistance. Treated jobseekers experienced an 8% increase in the probability of getting hired. Contrary to concerns that the assistance is taking away a valuable signal, we find no evidence that employers were less satisfied. We present a model in which better writing is not a signal of ability but helps employers ascertain ability, which rationalizes our findings.

==> Makefile <==
project_name = grammarly
public_name = algo_writing_assistance

ts := $(shell /bin/date "+%Y-%m-%d---%H-%M-%S")

package_list.txt:
	 find ../analysis/ -name *R -print0 | xargs -0 grep -h 'library*' | sed 's/library//g' | sed 's/#//g' | sed 's/ //g' | sort | uniq| sed 's/(//g' | sed 's/)//g' > package_list.txt

install_packages: package_list.txt
	cat package_list.txt | xargs -I {} Rscript -e 'install.packages("{}")'

#=================
##  DATA
#=================

# ---- raw data sets
allocations = ../etl/data/allocations.csv
freelancer_raw = ../etl/data/freelancer.csv
invites = ../etl/data/invites.csv
interviews = ../etl/data/interviews.csv
hires = ../etl/data/hires.csv
applications = ../etl/data/applications.csv

# ---- auxiliary files and data sets
input = ../analysis/input.R

freelancer = ../computed_objects/freelancer.csv
spell_check  =../computed_objects/spell_check.rds
spell_check_languagetool = ../computed_objects/spell_check_languagetool.rds
main_outcomes = ../computed_objects/main_outcomes.rds
writing_outcomes = ../computed_objects/writing_outcomes.rds

mechanism = ../computed_objects/mechanism.rds
quantiles = ../computed_objects/quantiles.rds


params =

tables =

#=================
## 0. AUXILIARY
#=================

##################
## preprocessing
##################

## --- 1. Get profiles spell checked
# compute
../computed_objects/spell_check.rds: ../analysis/spell_check.R $(input) $(freelancer_raw)
	cd ../analysis && Rscript spell_check.R

## --- 2. Create freelancer dataset
# compute
../computed_objects/freelancer.csv: ../analysis/co_freelancer.R $(input) $(freelancer_raw) $(spell_check)
	cd ../analysis && Rscript co_freelancer.R

## --- 3. Compute main outcomes
# compute
../computed_objects/main_outcomes.rds: ../analysis/co_main_outcomes.R $(input) $(freelancer) $(invites) $(interviews) $(hires) $(spell_check)
	cd ../analysis && Rscript co_main_outcomes.R

## --- 4. Compute mechanism outcomes
# compute
../computed_objects/mechanism.rds: ../analysis/co_mechanism.R $(input) $(freelancer) $(invites) $(interviews) $(hires)
	cd ../analysis && Rscript co_mechanism.R

## --- 4. Compute quantiles
# compute
../computed_objects/quantiles.rds: ../analysis/co_quantiles.R $(input) $(spell_check)
	cd ../analysis && Rscript co_quantiles.R

## --- 5. Compute writing outcomes
# compute
../computed_objects/writing_outcomes.rds: ../analysis/co_writing_outcomes.R $(input) $(freelancer) $(spell_check)
	cd ../analysis && Rscript co_writing_outcomes.R

##################
## parameters
##################

## --- 1. Compute general params
# compute
params += parameter_files/parameters.tex
parameter_files/parameters.tex: ../analysis/parameters.R $(input) $(freelancer) $(invites) $(interviews) $(hires)
	cd ../analysis && Rscript parameters.R

../computed_objects/spell_check_languagetool.rds:
	cp ~/Dropbox/data_for_sharing/grammarly/spell_check_languagetool.rds ../computed_objects/

#=================
## 1. ANALYSIS
#=================

tables += tables/hiring.tex
tables/hiring.tex: ../analysis/table_hiring.R $(input) $(freelancer)
	cd ../analysis && Rscript table_hiring.R

tables += tables/balance.tex
tables/balance.tex: ../analysis/table_balance.R $(input) $(freelancer)
	cd ../analysis && Rscript table_balance.R

tables += tables/predict_hiring_languagetool.tex
tables/predict_hiring_languagetool.tex: ../analysis/table_predict_hiring_languagetool.R $(input) $(freelancer) $(spell_check) $(spell_check_languagetool) $(invites) $(interviews) $(hires) ../computed_objects/spell_check.rds
	cd ../analysis && Rscript table_predict_hiring_languagetool.R

tables += tables/predict_hiring_languagetool_perword.tex
tables/predict_hiring_languagetool_perword.tex: ../analysis/table_predict_hiring_languagetool_perword.R $(input) $(freelancer) $(spell_check) $(spell_check_languagetool) $(invites) $(interviews) $(hires) ../computed_objects/spell_check.rds
	cd ../analysis && Rscript table_predict_hiring_languagetool_perword.R

tables += tables/predict_hiring_languagetool_total.tex
tables/predict_hiring_languagetool_total.tex: ../analysis/table_predict_hiring_languagetool_total.R $(input) $(freelancer) $(spell_check) $(spell_check_languagetool) $(invites) $(interviews) $(hires)
	cd ../analysis && Rscript table_predict_hiring_languagetool_total.R

tables += tables/summary_languagetool_error.tex
tables/summary_languagetool_error.tex: ../analysis/table_summary_languagetool_error.R $(input) $(freelancer) $(spell_check) $(spell_check_languagetool) $(invites) $(interviews) $(hires) ../computed_objects/spell_check_languagetool.rds
	cd ../analysis && Rscript table_summary_languagetool_error.R

tables += tables/summary_stats_pre.tex
tables/summary_stats_pre.tex: ../analysis/table_summary_stats.R $(input) $(freelancer)
	cd ../analysis && Rscript table_summary_stats.R

tables += tables/summary_stats_post.tex
tables/summary_stats_post.tex: ../analysis/table_summary_stats.R $(input) $(freelancer)
	cd ../analysis && Rscript table_summary_stats.R


tables += tables/writing_outcomes_1.tex
tables/writing_outcomes_1.tex: ../analysis/table_writing_outcomes.R $(input) $(freelancer) $(spell_check) $(spell_check_languagetool)
	cd ../analysis && Rscript table_writing_outcomes.R

tables += tables/writing_outcomes_2.tex
tables/writing_outcomes_2.tex: ../analysis/table_writing_outcomes.R $(input) $(freelancer) $(spell_check) $(spell_check_languagetool)
	cd ../analysis && Rscript table_writing_outcomes.R


tables += tables/main_outcomes.tex
tables/main_outcomes.tex: ../analysis/table_main_outcomes.R $(input) $(freelancer) $(invites) $(interviews) $(hires)
	cd ../analysis && Rscript table_main_outcomes.R

tables += tables/main_outcomes_uncon.tex
tables/main_outcomes_uncon.tex: ../analysis/robustness_checks.R $(input) $(freelancer) $(hires) $(invites) $(interviews)
	cd ../analysis && Rscript robustness_checks.R

tables += tables/main_outcomes_control.tex
tables/main_outcomes_control.tex: ../analysis/robustness_checks.R $(input) $(freelancer) $(hires) $(invites) $(interviews)
	cd ../analysis && Rscript robustness_checks.R

tables += tables/treatment.tex
tables/treatment.tex: ../analysis/table_treatment.R $(input) $(freelancer) $(spell_check) ../computed_objects/spell_check.rds
	cd ../analysis && Rscript table_treatment.R


tables += tables/applications.tex
tables/applications.tex: ../analysis/table_applications.R $(input) $(freelancer) $(applications)
	cd ../analysis && Rscript table_applications.R

tables += tables/length.tex
tables/length.tex: ../analysis/table_length.R $(input) $(freelancer) $(spell_check)
	cd ../analysis && Rscript table_length.R

tables += tables/approved.tex
tables/approved.tex: ../analysis/table_approved.R $(input) $(freelancer)
	cd ../analysis && Rscript table_approved.R

tables += tables/submitted.tex
tables/submitted.tex: ../analysis/table_submitted.R $(input) $(freelancer)
	cd ../analysis && Rscript table_submitted.R

tables += tables/wages_and_rates.tex
tables/wages_and_rates.tex: ../analysis/table_wages_and_rates.R $(input) $(freelancer) $(hires)
	cd ../analysis && Rscript table_wages_and_rates.R


plots += plots/allocations.pdf
plots/allocations.pdf: ../analysis/allocations.R $(input) $(allocations)
	cd ../analysis && Rscript allocations.R

plots += plots/bootstrap_sample_distro_of_marginal_rating.pdf
plots/bootstrap_sample_distro_of_marginal_rating.pdf: ../analysis/bootstrap_sample_distro_of_marginal_rating.R
	cd ../analysis && Rscript bootstrap_sample_distro_of_marginal_rating.R

plots += plots/main_outcomes.pdf
plots/main_outcomes.pdf: ../analysis/plot_main_outcomes.R $(input) $(main_outcomes)
	cd ../analysis && Rscript plot_main_outcomes.R

plots += plots/treatment.pdf
plots/treatment.pdf: ../analysis/plot_treatment.R $(input) $(main_outcomes)
	cd ../analysis && Rscript plot_treatment.R

plots += plots/approved.pdf
plots/approved.pdf: ../analysis/plot_approved.R $(input) $(main_outcomes)
	cd ../analysis && Rscript plot_approved.R

plots += plots/jss.pdf
plots/jss.pdf: ../analysis/jss.R $(input) $(main_outcomes)
	cd ../analysis && Rscript jss.R

plots += plots/mechanism.pdf
plots/mechanism.pdf: ../analysis/plot_mechanism.R $(input) $(mechanism)
	cd ../analysis && Rscript plot_mechanism.R

plots += plots/correlations.pdf
plots/correlations.pdf: ../analysis/plot_correlations.R $(input) $(freelancer) $(spell_check) $(invites) $(interviews) $(hires)
	cd ../analysis && Rscript plot_correlations.R

plots += plots/quantiles.pdf
plots/quantiles.pdf: ../analysis/plot_quantiles.R $(input) $(quantiles) $(spell_check)
	cd ../analysis && Rscript plot_quantiles.R

plots += plots/dag.pdf
plots/dag.pdf: ../analysis/dag.R $(input)
	cd ../analysis && Rscript dag.R

plots += plots/writing_outcomes.pdf
plots/writing_outcomes.pdf: ../analysis/plot_writing_outcomes.R $(input) $(writing_outcomes)
	cd ../analysis && Rscript plot_writing_outcomes.R

$(project_name).pdf : $(project_name).tex $(project_name).bib  $(tables) $(plots) $(params)
	#echo "\\\\newcommand{\\showCode}{false}" > show_code_params.tex
	pdflatex -shell-escape -interaction=batchmode $(project_name)
	pdflatex -shell-escape -interaction=batchmode $(project_name)
	bibtex $(project_name)
	pdflatex -shell-escape -interaction=batchmode $(project_name)
	pdflatex -shell-escape  -interaction=batchmode $(project_name)
	cp $(project_name).pdf $(project_name)_with_code.pdf
	gs -q -dNOPAUSE -dBATCH -dPDFSETTINGS=/prepress -sDEVICE=pdfwrite -sOutputFile=tmp.pdf $(project_name).pdf
	pdftk $(project_name).pdf cat 1-38 39-41east output $(project_name)_rotated.pdf
	mv $(project_name).pdf $(project_name)_unrotated.pdf
	cp $(project_name)_rotated.pdf $(project_name).pdf 

.PHONY: clean

clean:
	rm *.blg
	rm *.bbl
	rm *.aux
	rm *.out
	rm *.log
	rm *.pdf
	rm *.ttt
	rm *.fff
	rm *.lot
	rm *.log
	rm *.lof

.PHONY: website_without_code website_with_code

website_without_code: $(project_name).pdf
	printf 'cd papers\nput $<\n' \ | sftp -oPort=2222 johnjhorton@john-joseph-horton.com

website_with_code: $(project_name)_with_code.pdf
	printf 'cd papers\nput $<\n' \ | sftp -oPort=2222 johnjhorton@john-joseph-horton.com


website: $(project_name).pdf
	#make website_without_code
	#make website_with_code
	scp $(project_name).pdf johnjhorton@johnjhorton.ssh.wpengine.net:/home/wpe-user/sites/johnjhorton/papers/$(public_name).pdf


 ../backups/$(project_name)_$(ts).tar.gz:
	tar --exclude='../backups' --exclude='../analysis/py3env' --exclude='../surveys/code/ve3.5' --exclude='../.git' -zcvf ../backups/$(project_name)_$(ts).tar.gz ../


backup: ../backups/$(project_name)_$(ts).tar.gz
	echo "Creating backup"

backup_cloud: ../backups/$(project_name)_$(ts).tar.gz
	scp ../backups/$(project_name)_$(ts).tar.gz cloud:/shares/NAS

toread: $(project_name).pdf
	#scp $(project_name).pdf bandit:/home/ubuntu/Dropbox/toread/$(project_name)_$(ts).pdf
	#scp $(project_name).pdf bandit-local.local:/home/ubuntu/Dropbox/toread/$(project_name)_$(ts).pdf
	scp $(project_name).pdf ~/Dropbox/toread/$(project_name)_$(ts).pdf

cloud_backup: ../backups/$(project_name)_$(ts).tar.gz
	scp ../backups/$(project_name)_$(ts).tar.gz cloud:/shares/NAS

s3_backup: ../backups/$(project_name)_$(ts).tar.gz
	aws s3 cp ../backups/$(project_name)_$(ts).tar.gz s3://john_horton_backups/$(project_name)/

snapshot:
	@echo Timestamp is $(ts)
	cp $(project_name).pdf ../snapshots/$(project_name)_$(ts).pdf

purge:
	-cd plots && mv *pdf *png *svg unused/
	-cd tables && mv *tex unused/
	-cd ../computed_objects && mv *rds unused/

.PHONY: plots

plots:
	$(info $$var is [${plots}])


==> tables/balance.tex <==

% Table created by stargazer v.5.2.3 by Marek Hlavac, Social Policy Institute. E-mail: marek.hlavac at gmail.com
% Date and time: Thu, Jan 19, 2023 - 08:13:05 AM
\begin{table}[!htbp] \centering 
  \caption{Pre-randomization jobseeker attributes by cell} 
  \label{} 
\begin{tabular}{@{\extracolsep{5pt}} ccccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
Variable & Control & Treatment & Difference & P\_value \\ 
\hline \\[-1.8ex] 
From English-speaking country & $0.227$ & $0.227$ & $0.0003$ & $0.830$ \\ 
US-based & $0.185$ & $0.185$ & $0.0003$ & $0.789$ \\ 
Specializing in software & $0.077$ & $0.078$ & $0.001$ & $0.142$ \\ 
Specializing in writing & $0.132$ & $0.132$ & $0$ & $0.186$ \\ 
\end{tabular}
\hrule \emph{Notes:} This table shows the difference between treatment and control workers for means of pre-experiment covariates, as well as a t-test comparing the difference between those means.
\end{table}


==> tables/submitted.tex <==

\begin{table}[!htbp] \centering 
  \caption{Effects of writing assistance on worker profile submission rate} 
  \label{tab:submitted} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{1}{c}{\textit{Dependent variable:}} \\ 
\cline{2-2} 
\\[-1.8ex] & Profile Submitted x 100 \\ 
\hline \\[-1.8ex] 
 Algo Writing Treatment & 0.106 \\ 
  & (0.144) \\ 
  Constant & 45.532$^{***}$ \\ 
  & (0.102) \\ 
 \hline \\[-1.8ex] 
Observations & 480,948 \\ 
R$^{2}$ & 0.00000 \\ 
\hline 
\hline \\[-1.8ex] 
\end{tabular}
\\
\begin{minipage}{0.7 \textwidth}
{\footnotesize \emph{Notes}: 
          This table analyzes the effect of the treatment on 100 times a binary indicator for whether or not a jobseeker finished submitting their resume. 
          The sample is made up of all jobseekers in the experimental sample.
          \starlanguage}
\end{minipage}
\end{table}

